On Interpretations of Normal Modal Logics

We study interpretations of modal logics in one another where the Boolean connectives are interpreted identically and the modal operator diamond is interpreted by an arbitrary formula A(p). Clearly, such a formula A(p) defines an interpretation of a normal modal logic whenever A(p) is additive (that is, preserves disjunction) and normal (that is, preserves bottom) in the target logic. In the present paper, we provide a complete description of all additive and normal formulas in five prominent modal logics: K, GL, Grz, S4, and S5. For K, GL, and S5, we also describe all additive and normal formulas with parameters.

==> eptcsdata.tex <==
\providecommand{\firstpage}{321}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.18}{10.4204/EPTCS.447.18}}

